MusculoSkeletal Modeling Using Kinect Data For Telerehabilitation

Balance, gait and postural control are some of the key factors in determining the overall stability of an individual. Several highend and costly solutions exist to perform movement analysis in clinical settings. OpenSim is a tool which uses 39 marker positions, obtained from such highend solutions like VICON or equivalent multicamera setup, for the analysis of inverse kinematics and inverse dynamics. However, an affordable solution for deriving musculoskeletal joint kinematics parameters using a low cost Kinect device is of immense importance. In this paper, we initially study the feasibility of using OpenSim tool on 20 joint locations of human being, obtained from Kinect data. Next, we analyze the various joint forces and torques experienced during a Single Limb Stance (SLS) exercise performed by healthy subjects in normal, overweight and obese categories. Results indicate that a subset of parameters related to forces and torque in hip, lumber and pelvis are the most important ones that contribute significantly in maintaining static balance in SLS. Statistical analysis demonstrates that the pelvis list and tilt moments are the key biomarkers for maintaining the statibility in SLS, thus leading to a possibility of personalizing the therapy in tele-rehabilitation.

==> nipsOrg.tex <==
@inproceedings{kot2014modeling,
  title={Modeling of human balance as an inverted pendulum},
  author={Kot, Andrzej and Nawrocka, Agata},
  booktitle={Control Conference (ICCC), 2014 15th International Carpathian},
  pages={254--257},
  year={2014},
  organization={IEEE}
}

@article{winter1998stiffness,
  title={Stiffness control of balance in quiet standing},
  author={Winter, David A and Patla, Aftab E and Prince, Francois and Ishac, Milad and Gielo-Perczak, Krystyna},
  journal={Journal of neurophysiology},
  volume={80},
  number={3},
  pages={1211--1221},
  year={1998},
  publisher={Am Physiological Soc}
}

@article{winter1995human,
  title={Human balance and posture control during standing and walking},
  author={Winter, David A},
  journal={Gait \& posture},
  volume={3},
  number={4},
  pages={193--214},
  year={1995},
  publisher={Elsevier}
}

@phdthesis{stimac1999standup,
  title={Standup and stabilization of the inverted pendulum},
  author={Stimac, Andrew K},
  year={1999},
  school={Massachusetts Institute of Technology}
}

@article{pinter2008dynamics,
  title={The dynamics of postural sway cannot be captured using a one-segment inverted pendulum model: a PCA on segment rotations during unperturbed stance},
  author={Pinter, Ilona J and Van Swigchem, Roos and van Soest, AJ Knoek and Rozendaal, Leonard A},
  journal={Journal of neurophysiology},
  volume={100},
  number={6},
  pages={3197--3208},
  year={2008},
  publisher={Am Physiological Soc}
}
@article{orin2013centroidal,
  title={Centroidal dynamics of a humanoid robot},
  author={Orin, David E and Goswami, Ambarish and Lee, Sung-Hee},
  journal={Autonomous Robots},
  volume={35},
  number={2-3},
  pages={161--176},
  year={2013},
  publisher={Springer}
}

@article{dutta2010human,
  title={Human postural model that captures rotational inertia},
  author={Dutta, Anirban and Goswami, Ambarish},
  journal={American Society of Biomechanics, Providence, RI},
  year={2010}
}

@article{delp2007opensim,
  title={OpenSim: open-source software to create and analyze dynamic simulations of movement},
  author={Delp, Scott L and Anderson, Frank C and Arnold, Allison S and Loan, Peter and Habib, Ayman and John, Chand T and Guendelman, Eran and Thelen, Darryl G},
  journal={IEEE transactions on biomedical engineering},
  volume={54},
  number={11},
  pages={1940--1950},
  year={2007},
  publisher={IEEE}
}

@inproceedings{jun2003comparativeKinect,
  title={A Comparative Study of Human Motion Capture and Computational Analysis Tools},
  author={Jun, Seung-kook and Zhou, Xiaobo and Ramsey, Daniel K and Krovi, Venkat N},
  booktitle={The 2nd International Digital Human Modeling Symposium},
  year={2003},
  organization={Citeseer}
}

@article{delp2000computationalSIMM,
  title={A computational framework for simulating and analyzing human and animal movement},
  author={Delp, Scott L and Loan, J Peter},
  journal={Computing in Science \& Engineering},
  volume={2},
  number={5},
  pages={46--55},
  year={2000},
  publisher={AIP Publishing}
}
